Cryptocurrency with Fully Asynchronous Communication based on Banks and Democracy

Cryptocurrencies came to the world in the recent decade and attempted to offer a new order where the financial system is not governed by a centralized entity, and where you have complete control over your account without the need to trust strangers (governments and banks above all). However, cryptocurrency systems face many challenges that prevent them from being used as an everyday coin. In this paper we attempt to take one step forward by introducing a cryptocurrency system that has many important properties. Perhaps the most revolutionary property is its deterministic operation over a fully asynchronous communication network, which has sometimes been mistakenly considered to be impossible. By avoiding any temporal assumptions, we get a system that is robust against arbitrary delays in the network, and whose latency is only a function of the actual communication delay. The presented system is based on familiar concepts $-$ banking and democracy. Our banks, just like normal banks, keep their clients' money and perform their clients' requests. However, because of the cryptographic scheme, your bank cannot do anything in your account without your permission and its entire operation is transparent so you don't have to trust it blindly. The democracy means that every operation performed by the banks (e.g., committing a client transaction) has to be accepted by a majority of the coin holders, in a way that resembles representative democracy where the banks are the representatives and where each client implicitly delegates his voting power (the sum of money in his account) to his bank. A client can switch banks at any moment, by simply applying a corresponding request to the new bank of his choice.

==> Add-ons.tex <==
% !TEX root = Main.tex
% Add-ons

In this section additional options and features are presented.
is is beyond the scope here. 

\subsection{Partial-synchronous}
In the asynchronous settings we assume that less than one third of the voting power is in malicious hands.
If we assume some sort of synchronous, where there is an upper bound on the time it takes a message that was sent by a valid bank to reach another valid bank, then the system can be secured against even bigger proportion of malicious voting power.
Under such settings, when a valid bank receives a node from another bank, it can send this node to all other banks, and then wait that upper bound on messages transmission time (twice) to make sure that no other valid bank has received a conflicting node.
Only then it adds the received node to its graph.
%If it receives also a conflicting node during this period, then it adds both nodes at once

\subsection{Practical}

A final word concerning the small latency: Note that the communication between banks is a direct communication - each bank should know the IP of the other banks.
This is not a must (there is no importance from where a message signed by another bank has been received, as long as it is properly signed), but it can save important time, and there is no reason why it won't be that way.

Courtesy among banks:
1) if you supported a block of another bank, wait for it to acknowledge this support before you support a newer block of its. 
This is important to not giving legitimacy for ``satellite'' banks, that support only a specific (probably malicious) bank.
2) a ``smaller'' bank should first support a bigger bank's block.
Small banks issue: 


\subsection{Forking}
* when graphs diverge
* when banks cannot make advancement due to non-responding or ignoring banks.



However, it is still recommended to combine it with other existing ideas of reducing the load by using ``side channels'' to perform frequent and small money transfers (micro-payments), see e.g. \cite{lightning}.

